Learning logic programs by explaining their failures

Scientists form hypotheses and experimentally test them. If a hypothesis fails (is refuted), scientists try to explain the failure to eliminate other hypotheses. The more precise the failure analysis the more hypotheses can be eliminated. Thus inspired, we introduce failure explanation techniques for inductive logic programming. Given a hypothesis represented as a logic program, we test it on examples. If a hypothesis fails, we explain the failure in terms of failing sub-programs. In case a positive example fails, we identify failing sub-programs at the granularity of literals. We introduce a failure explanation algorithm based on analysing branches of SLD-trees. We integrate a meta-interpreter based implementation of this algorithm with the test-stage of the Popper ILP system. We show that fine-grained failure analysis allows for learning fine-grained constraints on the hypothesis space. Our experimental results show that explaining failures can drastically reduce hypothesis space exploration and learning times.

==> 00-declarations.tex <==
\section{Declarations}

%>>Author must provide "Declarations" to be placed just before references. (If any of section is not relevant to your manuscript write "Not Applicable")
\paragraph{Funding}

%(information that explains whether and by whom the research was supported)
Rolf Morel was supported by the Engineering and Physical Sciences Research Council (EP/N509711/1).
Andrew Cropper was supported by the EPSRC fellowship The Automatic Computer Scientist (EP/V040340/1).

\paragraph{Conflicts of interest/Competing interests}
%(include appropriate disclosures)
Not applicable.

\paragraph{Ethics approval}
%(include appropriate approvals or waivers)
Not applicable.

\paragraph{Consent to participate}
%(include appropriate consent statements)
Not applicable.

\paragraph{Consent for publication}
%(appropriate statements regarding publishing an individual’s data or image)
Not applicable.

\paragraph{Availability of data and material}
%(data transparency)
Upon publication, all datasets and experimental code will be made freely available on a public repository.

\paragraph{Code availability}
%(software application or custom code)
Upon publication, the software for this project, i.e.~the implementation of \name{}, will be made freely available on a public repository.

\paragraph{Authors' contributions}
%(all authors must mentioned in the statement)
Rolf Morel was the main investigator of the research in this manuscript.
Rolf developed the algorithm(s), implemented the ILP system described, and wrote the experimental code.
Rolf wrote each section.
Andrew Cropper supervised the project.
Andrew proposed the overall structure, suggested how to frame the algorithm(s), adviced on experimental setup, and went through the document as an editor a number of times.


==> 05-05-iggp.tex <==
\subsection{Experiment 5: IGGP}

some text
\begin{table}[ht]
\scriptsize
\centering
\begin{tabular}{
\narrowc
\narrowc|\narrowc
\narrowc|\narrowc
}
%\toprule
\multicolumn{1}{c}{} &
\multicolumn{2}{c}{\textbf{Learning time}} &
\multicolumn{2}{c}{\textbf{Accuracy}} \\

%\toprule
\cmidrule(r){2-3}
\cmidrule(r){4-5}
% \cmidrule{2-4} \cmidrule{6-7} \\
% \addlinespace[10pt]
\textbf{Problem} &
\nameold{} & \name{} & \nameold{} & \name{} \\
\cmidrule(lr){1-1}
\cmidrule(r){2-3}
\cmidrule(r){4-5}
minimal-decay &
90 $\pm$ 0.0 & 42 $\pm$ 4 & 0.9 $\pm$ 0.0 & 1.0 $\pm$ 0.0 \\
rps &
90 $\pm$ 0.0 & 26 $\pm$ 1 & 0.9 $\pm$ 0.0 & 1.0 $\pm$ 0.0 \\
coins &
90 $\pm$ 0.0 & 90 $\pm$ 0.2 & 0.8 $\pm$ 0.0 & 0.8 $\pm$ 0.0 \\
buttons &
90 $\pm$ 0.2 & 90 $\pm$ 0.2 & 0.9 $\pm$ 0.01 & 0.9 $\pm$ 0.01 \\
%
%dropk &
%251 $\pm$ 77 & 74 $\pm$ 35 & 0.30 &
%2 $\pm$ 0.9 & 2 $\pm$ 0.8 & 0.87 & N/A \\
%
%droplast &
%677 $\pm$ 724 & 554 $\pm$ 533 & 0.82 &
%8 $\pm$ 8 & 10 $\pm$ 8 & 1.31 & N/A \\
%
%evens &
%302 $\pm$ 7 & 264 $\pm$ 21 & 0.87 &
%4 $\pm$ 0.2 & 4 $\pm$ 0.4 & 1.07 & 54 $\pm$ 16 \\
%
%finddup &
%1164 $\pm$ 63 & 635 $\pm$ 52 & 0.55 &
%11 $\pm$ 1 & 7 $\pm$ 0.7 & 0.64 & 2 $\pm$ 1 \\
%
%last &
%226 $\pm$ 31 & 56 $\pm$ 28 & 0.25 &
%1 $\pm$ 0.2 & 0.7 $\pm$ 0.3 & 0.58 & 0.9 $\pm$ 0.7 \\
%
%len &
%594 $\pm$ 28 & 71 $\pm$ 15 & 0.12 &
%5 $\pm$ 0.4 & 1.0 $\pm$ 0.2 & 0.21 & 60 $\pm$ 0.1 \\
%
%member &
%58 $\pm$ 8 & 14 $\pm$ 3 & 0.25 &
%0.4 $\pm$ 0.0 & 0.3 $\pm$ 0.0 & 0.69 & 0.3 $\pm$ 0.0 \\
%
%sorted &
%767 $\pm$ 152 & 583 $\pm$ 125 & 0.76 &
%17 $\pm$ 5 & 16 $\pm$ 5 & 0.94 & 60 $\pm$ 0.0 \\
%
%threesame &
%24 $\pm$ 8 & 26 $\pm$ 8 & 1.08 &
%0.2 $\pm$ 0.1 & 0.3 $\pm$ 0.1 & 1.50 & 0.3 $\pm$ 0.2 \\




%len &
%590 $\pm$ 4 & 60 $\pm$ 5 & \textbf{0.10} &
%16 $\pm$ 0.2 & 1 $\pm$ 0.1 & \textbf{0.09} & 120 $\pm$ 0 \\
%
%dropk &
%114 $\pm$ 0.7 & 13 $\pm$ 1 & \textbf{0.12} &
%1 $\pm$ 0.01 & 0.3 $\pm$ 0.02 & \textbf{0.23} & N/A \\
%
%finddup &
%1223 $\pm$ 22 & 644 $\pm$ 14 & \textbf{0.53} &
%53 $\pm$ 2 & 20 $\pm$ 0.7 & \textbf{0.38} & 2 $\pm$ 0.4 \\
%
%member &
%57 $\pm$ 2 & 14 $\pm$ 0.7 & \textbf{0.24} &
%0.6 $\pm$ 0.03 & 0.2 $\pm$ 0.01 & \textbf{0.41} & 0.2 $\pm$ 0.01 \\
%
%last &
%232 $\pm$ 6 & 64 $\pm$ 6 & \textbf{0.28} &
%3 $\pm$ 0.1 & 2 $\pm$ 0.1 & \textbf{0.48} & 0.5 $\pm$ 0.05 \\
%
%evens &
%306 $\pm$ 2 & 278 $\pm$ 2 & \textbf{0.91} &
%7 $\pm$ 0.06 & 7 $\pm$ 0.09 & \textbf{1.00} & 112 $\pm$ 5 \\
%
%threesame &
%18 $\pm$ 4 & 15 $\pm$ 3 & \textbf{0.81} &
%0.2 $\pm$ 0.04 & 0.2 $\pm$ 0.04 & \textbf{1.00} & 0.3 $\pm$ 0.03 \\
%
%droplast &
%161 $\pm$ 9 & 148 $\pm$ 10 & \textbf{0.92} &
%11 $\pm$ 0.9 & 11 $\pm$ 1 & 1.02 & N/A \\
%
%addhead &
%32 $\pm$ 3 & 31 $\pm$ 2 & \textbf{0.96} &
%0.6 $\pm$ 0.04 & 0.6 $\pm$ 0.04 & 1.05 & N/A \\
%
%sorted &
%708 $\pm$ 40 & 599 $\pm$ 26 & \textbf{0.85} &
%29 $\pm$ 3 & 31 $\pm$ 2 & 1.08 & 119.27{$\pm$}0.8 \\

%\bottomrule
\cmidrule(lr){1-1}
\cmidrule(r){2-3}
\cmidrule(r){4-5}
\end{tabular}
\caption{
Programming puzzles results for \name{}, \nameold{} and \metagol{}.
Left, the average number of programs generated by each system.
Right, the (corresponding) average time to find a solution.
The error is standard error.
We round values over one to the nearest integer.
Values under one we round to the most significant digit.
}
\label{tab:puzzles}
\end{table}

%\begin{tabular}
%\end{tabular}

